DivaTrack: Diverse Bodies and Motions from Acceleration-Enhanced Three-Point Trackers

Full-body avatar presence is crucial for immersive social and environmental interactions in digital reality. However, current devices only provide three six degrees of freedom (DOF) poses from the headset and two controllers (i.e. three-point trackers). Because it is a highly under-constrained problem, inferring full-body pose from these inputs is challenging, especially when supporting the full range of body proportions and use cases represented by the general population. In this paper, we propose a deep learning framework, DivaTrack, which outperforms existing methods when applied to diverse body sizes and activities. We augment the sparse three-point inputs with linear accelerations from Inertial Measurement Units (IMU) to improve foot contact prediction. We then condition the otherwise ambiguous lower-body pose with the predictions of foot contact and upper-body pose in a two-stage model. We further stabilize the inferred full-body pose in a wide range of configurations by learning to blend predictions that are computed in two reference frames, each of which is designed for different types of motions. We demonstrate the effectiveness of our design on a large dataset that captures 22 subjects performing challenging locomotion for three-point tracking, including lunges, hula-hooping, and sitting. As shown in a live demo using the Meta VR headset and Xsens IMUs, our method runs in real-time while accurately tracking a user's motion when they perform a diverse set of movements.

==> 7_figureonly.tex <==
\begin{figure*}[ht]
  \centering
  \includegraphics[width=\linewidth]{figures/SOTAComp2.png}
  \caption{Qualitative comparison with AvatarPoser. The darker red color denotes a larger error. Our Model, DivaTrack, produces outputs closer to the ground truth for both static movements (left: hula-hoop, lunge, and sitting down) and various locomotion (right: running, moving backward, and moving a box) of subjects with different body shapes.}
  \label{fig:sotaqual}
\end{figure*}

\begin{figure*}[ht]
  \centering
\includegraphics[width=\linewidth]{figures/RefComp.png}
  \caption{Comparison of reference frame definitions. Left: for static movements with slight head jiggling, $R_{traj}$ can rotate fast, resulting in jitter and sliding. Right: for locomotion with uncorrelated head direction, $R_{proj}$ are directed irrelevant to the translation, producing wrong poses. Our blending method can generate high-quality motions by taking advantage of two reference frames.}
  \label{fig:refqual}
\end{figure*}

\begin{figure*}[ht]
  \centering
\includegraphics[width=\linewidth]{figures/ContComp.png}
  \caption{Comparison of contact probabilities as L-model condition. Foot contacts enable the L-model to generate motions that are underdetermined by 3-point signals (i.e. kicking) and to maintain accurate footsteps while changing speed and direction.}
  \label{fig:contqual}
\end{figure*}

\begin{figure*}[ht]
  \centering
\includegraphics[width=\linewidth]{figures/IMUComp2.png}
  \caption{Comparison of acceleration sources. IMU accelerations help UC-Model predict accurate contacts for corner cases (left: lunge and right: carrying object), thereby allowing L-Model to generate high-quality lower-body motions with minimized sliding artifacts.}
  \label{fig:imuqual}
\end{figure*}
